Approximate Inference for Constructing Astronomical Catalogs from Images

We present a new, fully generative model for constructing astronomical catalogs from optical telescope image sets. Each pixel intensity is treated as a random variable with parameters that depend on the latent properties of stars and galaxies. These latent properties are themselves modeled as random. We compare two procedures for posterior inference. One procedure is based on Markov chain Monte Carlo (MCMC) while the other is based on variational inference (VI). The MCMC procedure excels at quantifying uncertainty, while the VI procedure is 1000 times faster. On a supercomputer, the VI procedure efficiently uses 665,000 CPU cores to construct an astronomical catalog from 50 terabytes of images in 14.6 minutes, demonstrating the scaling characteristics necessary to construct catalogs for upcoming astronomical surveys.

==> plots-s82/error_vb_mc_comparison.tex <==
\begin{tabular}{llll}
\toprule
{} &              MCMC &                VI &             Photo \\
\\midrule
direction    &  1.625 0.04 &  1.631 0.05 &  1.651 0.06 \\
flux   &  0.754 0.05 &  0.733 0.05 &  0.775 0.06 \\
color u-g    &  0.619 0.05 &  0.636 0.05 &  1.018 0.07 \\
color g-r    &  0.462 0.03 &  0.464 0.03 &  0.930 0.08 \\
color r-i    &  0.547 0.04 &  0.555 0.04 &  0.998 0.07 \\
color i-z    &  0.442 0.04 &  0.428 0.04 &  0.940 0.07 \\
galaxy profile      &  1.031 0.05 &  0.749 0.06 &  0.942 0.07 \\
galaxy axis         &  0.695 0.04 &  0.881 0.05 &  1.321 0.08 \\
galaxy radius       &  0.194 0.02 &  0.234 0.03 &  0.431 0.10 \\
galaxy angle        &  0.892 0.06 &  0.902 0.06 &  0.941 0.06 \\
\bottomrule
\end{tabular}


==> plots-s82/uscore_per.tex <==
\begin{tabular}{lrrrr}
{} &  &  \textbf{MCMC} &  & \\
\toprule
{} & within 1/2 sd & 1 sd & 2 sd & 3 sd \\
\midrule
log\_flux\_r &          0.18 & 0.37 & 0.65 & 0.82 \\
color ug   &          0.23 & 0.39 & 0.65 & 0.75 \\
color gr   &          0.32 & 0.56 & 0.83 & 0.94 \\
color ri   &          0.30 & 0.57 & 0.87 & 0.96 \\
color iz   &          0.30 & 0.56 & 0.87 & 0.97 \\
\bottomrule
\end{tabular}


==> plots-synthetic/uscore_mc.tex <==
\begin{tabular}{lrrrr}
{} &  &  \textbf{MCMC} &  & \\
\toprule
{} & within 1/2 sd &  1 sd &  2 sd &  3 sd \\
\midrule
log flux &         0.36 & 0.64 & 0.92 & 0.99 \\
color u-g   &         0.43 & 0.73 & 0.95 & 1.00 \\
color g-r   &         0.41 & 0.68 & 0.93 & 0.99 \\
color r-i   &         0.41 & 0.67 & 0.94 & 0.99 \\
color i-z   &         0.41 & 0.71 & 0.93 & 0.99 \\
\bottomrule
\end{tabular}

